How to Handle Assumptions in Synthesis

The increased interest in reactive synthesis over the last decade has led to many improved solutions but also to many new questions. In this paper, we discuss the question of how to deal with assumptions on environment behavior. We present four goals that we think should be met and review several different possibilities that have been proposed. We argue that each of them falls short in at least one aspect.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{K. Chatterjee, R. Ehlers, and S. Jha (Eds.): \\
Third Workshop on Synthesis (SYNT 2014)\\
EPTCS 157, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.157.7}{10.4204/EPTCS.157.7}}
\pdfoutput=1

